Particle Physics in the Sky and Astrophysics Underground: Connecting the Universe's Largest and Smallest Scales

Particles have tremendous potential as astronomical messengers, and conversely, studying the universe as a whole also teaches us about particle physics. This thesis encompasses both of these research directions. Many models predict a diffuse flux of high energy neutrinos from active galactic nuclei and other astrophysical sources. The "Astrophysics Underground" portion of this thesis describes a search for this neutrino flux performed by looking for very high energy upward-going muons using the Super-K detector. In addition to using particles to do astronomy, we can also use the universe itself as a particle physics lab. The "Particle Physics in the Sky" portion of this thesis focuses on extracting cosmological information from galaxy surveys. To overcome technical challenges faced by the latest galaxy surveys, we produced a comprehensive upgrade to mangle, a software package that processes the angular masks defining the survey area on the sky. We added dramatically faster algorithms and new useful features that are necessary for managing complex masks of current and next-generation galaxy surveys. With this software in hand, we utilized SDSS data to investigate the relation between galaxies and dark matter by studying relative bias, i.e., the relation between different types of galaxies. Separating galaxies by their luminosities and colors reveals a complicated picture: red galaxies are clustered more strongly than blue galaxies, with both the brightest and the faintest red galaxies showing the strongest clustering. Furthermore, red and blue galaxies tend to occupy different regions of space. In order to make precise measurements from the next generation of galaxy surveys, it will be essential to account for this complexity.

==> Acknowledgments_SK.tex <==
%auto-ignore
\section{Acknowledgments}
\label{sec:Acknowledgments}
We gratefully acknowledge the cooperation of the Kamioka Mining and
Smelting Company.  The Super-Kamiokande experiment has been built and
operated from funding by the Japanese Ministry of Education, Culture,
Sports, Science and Technology, the United States Department of Energy,
and the US National Science Foundation.
Some of us have been supported by funds from the Korean Research
Foundation (BK21) and the Korea Science and Engineering Foundation, 
the Polish Committee for Scientific Research (grant 1P03B08227),
Japan Society for the Promotion of Science, and
Research Corporation's Cottrell College Science Award.


==> authoraasstyle.tex <==
\def\icrr{1}
\def\ncen{2}
\def\bu{3}
\def\bnl{4}
\def\uci{5}
\def\csu{6}
\def\cnu{7}
\def\duke{8}
\def\gmu{9}
\def\gifu{10}
\def\uh{11}
\def\ui{12}
\def\kek{13}
\def\kobe{14}
\def\kyoto{15}
\def\lanl{16}
\def\lsu{17}
\def\umd{18}
\def\mit{19}
\def\duluth{20}
\def\miyagi{21}
%\def\nagoya{23}
\def\nagoyaste{22}
\def\suny{23}
\def\niigata{24}
\def\okayama{25}
\def\osaka{26}
\def\seoul{27}
%\def\shizuokaseika{28}
\def\shizuoka{28}
\def\shizuokafukushi{29}
\def\skku{30}
\def\tohoku{31}
\def\tokai{32}
\def\tit{33}
\def\tokyo{34}
\def\warsaw{35}
\def\uw{36}
%
%\def\corresponding{*}
%\def\pennnow{$\dagger$}
%\def\kamiokanow{$\ddagger$}
%\def\icrrnow{\S}
%\def\triumfnow{\P}
%\def\stanfordnow{$||$}
%\def\columbianow{**}
\def\corresponding{a}
\def\pennnow{b}
\def\kamiokanow{c}
\def\icrrnow{d}
\def\triumfnow{e}
\def\stanfordnow{f}
\def\columbianow{g}
%
%a hack so things don't take forever to latex
%\newcommand{\tempaltaffiltext}[1]{$^{#1}$}
%
\author{
%First author
M.E.C.~Swanson\altaffilmark{\mit,\corresponding},
%Kamioka observatory
K.~Abe\altaffilmark{\icrr}, %not in 3flavor - joined april 2005
J.~Hosaka\altaffilmark{\icrr},
T.~Iida\altaffilmark{\icrr},  %not in 3flavor - joined april 2005
K.~Ishihara\altaffilmark{\icrr},
J.~Kameda\altaffilmark{\icrr},
Y.~Koshio\altaffilmark{\icrr},
A.~Minamino\altaffilmark{\icrr},
C.~Mitsuda\altaffilmark{\icrr},
M.~Miura\altaffilmark{\icrr},
S.~Moriyama\altaffilmark{\icrr},
M.~Nakahata\altaffilmark{\icrr},
%T.~Namba\altaffilmark{\icrr}, %in 3flavor - expired Feb 2006
Y.~Obayashi\altaffilmark{\icrr},
H.~Ogawa\altaffilmark{\icrr},  %not in 3flavor - joined Oct 2004
M.~Shiozawa\altaffilmark{\icrr},
Y.~Suzuki\altaffilmark{\icrr},
A.~Takeda\altaffilmark{\icrr},
Y.~Takeuchi\altaffilmark{\icrr},
K.~Ueshima\altaffilmark{\icrr},  %not in 3flavor- joined april 2005 
%S.~Yamada\altaffilmark{\icrr}, %in 3flavor - expired april 2006
%
%Research center for cosmic neutrinos
I.~Higuchi\altaffilmark{\ncen},
C.~Ishihara\altaffilmark{\ncen}, %not in 3flavor - joined april 2005
M.~Ishitsuka\altaffilmark{\ncen},
T.~Kajita\altaffilmark{\ncen},
K.~Kaneyuki\altaffilmark{\ncen},
G.~Mitsuka\altaffilmark{\ncen},
S.~Nakayama\altaffilmark{\ncen},
H.~Nishino\altaffilmark{\ncen},
A.~Okada\altaffilmark{\ncen}, %in 3flavor - expired april 2006 but contributed to UHE analysis
K.~Okumura\altaffilmark{\ncen},
C.~Saji\altaffilmark{\ncen},
Y.~Takenaga\altaffilmark{\ncen},
%
%Boston U
S.~Clark\altaffilmark{\bu},
S.~Desai\altaffilmark{\bu,\pennnow},
F.~Dufour\altaffilmark{\bu},  %not in 3flavor - joined april 2005
E.~Kearns\altaffilmark{\bu},
S.~Likhoded\altaffilmark{\bu},
M.~Litos\altaffilmark{\bu}, %not in 3flavor - joined april 2005
J.L.~Raaf\altaffilmark{\bu}, %not in 3flavor - joined april 2005
J.L.~Stone\altaffilmark{\bu},
L.R.~Sulak\altaffilmark{\bu},
W.~Wang\altaffilmark{\bu},
%
%BNL
M.~Goldhaber\altaffilmark{\bnl},
%
%Irvine
D.~Casper\altaffilmark{\uci},
J.P.~Cravens\altaffilmark{\uci},
J.~Dunmore\altaffilmark{\uci},  %not in 3flavor - joined june 2004
W.R.~Kropp\altaffilmark{\uci},
D.W.~Liu\altaffilmark{\uci},
S.~Mine\altaffilmark{\uci},
C.~Regis\altaffilmark{\uci},
M.B.~Smy\altaffilmark{\uci},
H.W.~Sobel\altaffilmark{\uci},
%C.W.~Sterner\altaffilmark{\uci}, %in 3flavor - expired 0 2005 ???
M.R.~Vagins\altaffilmark{\uci},
%
%CSU
K.S.~Ganezer\altaffilmark{\csu},
J.E.~Hill\altaffilmark{\csu},
W.E.~Keig\altaffilmark{\csu},
%
%Chonnam National University
J.S.~Jang\altaffilmark{\cnu},
J.Y.~Kim\altaffilmark{\cnu},
I.T.~Lim\altaffilmark{\cnu},
%
%Duke
K.~Scholberg\altaffilmark{\duke,\mit},
N.~Tanimoto\altaffilmark{\duke},  %not in 3flavor - joined april 2005
C.W.~Walter\altaffilmark{\duke},
R.~Wendell\altaffilmark{\duke},  %not in 3flavor - not on ``all'' author list
%
%George Mason U
R.W.~Ellsworth\altaffilmark{\gmu},
%
%Gifu U
S.~Tasaka\altaffilmark{\gifu},
%Hawaii U
G.~Guillian\altaffilmark{\uh},
%A.~Kibayashi\altaffilmark{\uh}, %in 3flavor - expired oct 2005
J.G.~Learned\altaffilmark{\uh},
S.~Matsuno\altaffilmark{\uh},
%
%Indiana University
M.D.~Messier\altaffilmark{\ui},
%KEK
Y.~Hayato\altaffilmark{\kek,\kamiokanow},
A.K.~Ichikawa\altaffilmark{\kek},
T.~Ishida\altaffilmark{\kek},
T.~Ishii\altaffilmark{\kek},
T.~Iwashita\altaffilmark{\kek},
T.~Kobayashi\altaffilmark{\kek},
T.~Nakadaira\altaffilmark{\kek},
K.~Nakamura\altaffilmark{\kek},
K.~Nitta\altaffilmark{\kek},
Y.~Oyama\altaffilmark{\kek},
Y.~Totsuka\altaffilmark{\kek,\icrrnow},
%
%Kobe U
A.T.~Suzuki\altaffilmark{\kobe},
%
%Kyoto
M.~Hasegawa\altaffilmark{\kyoto},
K.~Hiraide\altaffilmark{\kyoto},  %not in 3flavor - joined april 2005
I.~Kato\altaffilmark{\kyoto,\triumfnow},
H.~Maesaka\altaffilmark{\kyoto},
T.~Nakaya\altaffilmark{\kyoto},
K.~Nishikawa\altaffilmark{\kyoto},
T.~Sasaki\altaffilmark{\kyoto},
H.~Sato\altaffilmark{\kyoto},
S.~Yamamoto\altaffilmark{\kyoto},
M.~Yokoyama\altaffilmark{\kyoto},
%
%Los Alamos
T.J.~Haines\altaffilmark{\lanl,\uci},
%
%LSU
S.~Dazeley\altaffilmark{\lsu},
S.~Hatakeyama\altaffilmark{\lsu},
R.~Svoboda\altaffilmark{\lsu},
%
%Maryland U
%E.~Blaufuss\altaffilmark{\umd}, %in 3flavor - expired april 2006
%J.A.~Goodman\altaffilmark{\umd}, %in 3flavor - expired april 2006
G.W.~Sullivan\altaffilmark{\umd},
D.~Turcan\altaffilmark{\umd},
%
% MIT
J.~Cooley\altaffilmark{\mit,\stanfordnow}, %in 3flavor -expired oct 2005 but contributed to UHE analysis
K.B.M.~Mahn\altaffilmark{\mit,\columbianow}, %MIT undergrad who contributed to UHE analysis
%
%University of Minnesota, Duluth
A.~Habig\altaffilmark{\duluth},
%
% Miyagi U. of Education
Y.~Fukuda\altaffilmark{\miyagi}, 
T.~Sato\altaffilmark{\miyagi}, 
%
%Nagoya U.
Y.~Itow\altaffilmark{\nagoyaste},
T.~Koike\altaffilmark{\nagoyaste}, %not in 3flavor - joined april 2005
%
%SUNY
C.K.~Jung\altaffilmark{\suny},
T.~Kato\altaffilmark{\suny},
K.~Kobayashi\altaffilmark{\suny},
M.~Malek\altaffilmark{\suny},
%C.~Mauger\altaffilmark{\suny}, %in 3flavor - expired dec 2005
C.~McGrew\altaffilmark{\suny},
A.~Sarrat\altaffilmark{\suny},
R.~Terri\altaffilmark{\suny}, %not in 3flavor - joined oct 2004
C.~Yanagisawa\altaffilmark{\suny},
%%
%Niigata U
N.~Tamura\altaffilmark{\niigata},
%
%Okayama U.
M.~Sakuda\altaffilmark{\okayama},
M.~Sugihara\altaffilmark{\okayama},%not in 3flavor - joined april 2005
%
%Osaka U.
Y.~Kuno\altaffilmark{\osaka},
M.~Yoshida\altaffilmark{\osaka},
%
%Seoul
S.B.~Kim\altaffilmark{\seoul},
B.S.~Yang\altaffilmark{\seoul},%not in 3flavor - joined march 2005
J.~Yoo\altaffilmark{\seoul},
%
%Shizuoka
T.~Ishizuka\altaffilmark{\shizuoka},
%
%Shizuoka seika
H.~Okazawa\altaffilmark{\shizuokafukushi}, 
%
%Sungkyunkwan University
Y.~Choi\altaffilmark{\skku},
H.K.~Seo\altaffilmark{\skku},
%
%Tohoku U.
Y.~Gando\altaffilmark{\tohoku},
T.~Hasegawa\altaffilmark{\tohoku},
K.~Inoue\altaffilmark{\tohoku},
%J.~Shirai\altaffilmark{\tohoku}, %in 3flavor - expired april 2006
%A.~Suzuki\altaffilmark{\tohoku}, %in 3flavor - expired april 2006
%
%Tokai U
H.~Ishii\altaffilmark{\tokai},%not in 3flavor - joined april 2005
K.~Nishijima\altaffilmark{\tokai},
%
%TIT
H.~Ishino\altaffilmark{\tit},
Y.~Watanabe\altaffilmark{\tit},
%
%Tokyo U
M.~Koshiba\altaffilmark{\tokyo},
%
%Warsaw U
D.~Kielczewska\altaffilmark{\warsaw,\uci},
J.~Zalipska\altaffilmark{\warsaw},
%U Washington
H.G.~Berns\altaffilmark{\uw},
R.~Gran\altaffilmark{\uw,\duluth},
K.K.~Shiraishi\altaffilmark{\uw},
A.~Stachyra\altaffilmark{\uw},%in 3flavor - expired dec 2005 but contributed to UHE analysis
E.~Thrane\altaffilmark{\uw},%not in 3flavor - joined oct 2004
K.~Washburn\altaffilmark{\uw},
and
R.J.~Wilkes\altaffilmark{\uw}\\
(The Super-Kamiokande Collaboration)\\
\footnotesize
\rm
\altaffiltext{\icrr}{Kamioka Observatory, Institute for Cosmic Ray Research, 
University of Tokyo, Kamioka, Gifu, 506-1205, Japan }
\altaffiltext{\ncen}{Research Center for Cosmic Neutrinos, Institute for Cosmic 
Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan }
\altaffiltext{\bu}{Department of Physics, Boston University, Boston, MA 02215, 
USA }
\altaffiltext{\bnl}{Physics Department, Brookhaven National Laboratory, Upton, 
NY 11973, USA }
\altaffiltext{\uci}{Department of Physics and Astronomy, University of 
California, Irvine, Irvine, CA 92697-4575, USA }
\altaffiltext{\csu}{Department of Physics, California State University, 
Dominguez Hills, Carson, CA 90747, USA }
\altaffiltext{\cnu}{Department of Physics, Chonnam National University, Kwangju 
500-757, Korea }
\altaffiltext{\duke}{Department of Physics,Duke University, Durham, NC 27708, USA }
\altaffiltext{\gmu}{Department of Physics, George Mason University, Fairfax, VA 
22030, USA }
\altaffiltext{\gifu}{Department of Physics, Gifu University, Gifu, Gifu 
501-1193, Japan }
\altaffiltext{\uh}{Department of Physics and Astronomy, University of Hawaii, 
Honolulu, HI 96822, USA }
\altaffiltext{\ui}{Department of Physics, Indiana University, Bloomington,
 IN 47405-7105, USA } 
\altaffiltext{\kek}{High Energy Accelerator Research Organization (KEK), 
Tsukuba, Ibaraki 305-0801, Japan }
\altaffiltext{\kobe}{Department of Physics, Kobe University, Kobe, Hyogo 
657-8501, Japan }
\altaffiltext{\kyoto}{Department of Physics, Kyoto University, Kyoto 606-8502, 
Japan }
\altaffiltext{\lanl}{Physics Division, P-23, Los Alamos National Laboratory, Los 
Alamos, NM 87544, USA }
\altaffiltext{\lsu}{Department of Physics and Astronomy, Louisiana State 
University, Baton Rouge, LA 70803, USA }
\altaffiltext{\umd}{Department of Physics, University of Maryland, College Park, 
MD 20742, USA }
\altaffiltext{\mit}{Department of Physics, Massachusetts Institute of 
Technology, Cambridge, MA 02139, USA }
\altaffiltext{\duluth}{Department of Physics, University of Minnesota, 
Duluth, MN 55812-2496, USA }
\altaffiltext{\miyagi}{Department of Physics, Miyagi University of Education, Sendai,Miyagi 980-0845, Japan }
%\altaffiltext{\nagoya}{Department of Physics, Nagoya University, Nagoya, Aichi 
%464-8602, Japan }
\altaffiltext{\nagoyaste}{Solar-Terrestrial Environment Laboratory, Nagoya University, Nagoya, Aichi 464-8601, Japan }
\altaffiltext{\suny}{Department of Physics and Astronomy, State University of 
New York, Stony Brook, NY 11794-3800, USA }
\altaffiltext{\niigata}{Department of Physics, Niigata University, Niigata, 
Niigata 950-2181, Japan }
\altaffiltext{\okayama}{Department of Physics, Okayama University, Okayama, Okayama 700-8530, Japan }
\altaffiltext{\osaka}{Department of Physics, Osaka University, Toyonaka, Osaka 
560-0043, Japan }
\altaffiltext{\seoul}{Department of Physics, Seoul National University, Seoul 
151-742, Korea }
%\altaffiltext{\shizuokaseika}{International and Cultural Studies, Shizuoka Seika College, Yaizu, Shizuoka, 425-8611, Japan }
\altaffiltext{\shizuoka}{Department of Systems Engineering, Shizuoka University, 
Hamamatsu, Shizuoka 432-8561, Japan }
\altaffiltext{\shizuokafukushi}{Department of Informatics in
Social Welfare, Shizuoka University of Welfare, Yaizu, Shizuoka 425-8611, Japan }
\altaffiltext{\skku}{Department of Physics, Sungkyunkwan University, Suwon 
440-746, Korea }
\altaffiltext{\tohoku}{Research Center for Neutrino Science, Tohoku University, 
Sendai, Miyagi 980-8578, Japan }
\altaffiltext{\tokai}{Department of Physics, Tokai University, Hiratsuka, 
Kanagawa 259-1292, Japan }
\altaffiltext{\tit}{Department of Physics, Tokyo Institute for Technology, 
Meguro, Tokyo 152-8551, Japan }
\altaffiltext{\tokyo}{The University of Tokyo, Tokyo 113-0033, Japan }
\altaffiltext{\warsaw}{Institute of Experimental Physics, Warsaw University, 
00-681 Warsaw, Poland }
\altaffiltext{\uw}{Department of Physics, University of Washington, Seattle, WA 
98195-1560, USA }
%end authors
}
\altaffiltext{\corresponding}{Electronic address: molly@space.mit.edu}
\altaffiltext{\pennnow}{Present address: Center for Gravitational Wave Physics, Pennsylvania State University, University Park, PA 16802, USA}
\altaffiltext{\kamiokanow}{Present address: Kamioka Observatory, Institute for Cosmic Ray Research, University of Tokyo, Kamioka, Gifu, 506-1205, Japan}
\altaffiltext{\icrrnow}{Present address: Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan}
\altaffiltext{\triumfnow}{Present address: TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\altaffiltext{\stanfordnow}{Present address: Department of Physics, Stanford University, Stanford, CA 94305, USA}
\altaffiltext{\columbianow}{Present address: Department of Physics, Columbia University, New York, NY 10027, USA}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> authorapjstyle.tex <==
%auto-ignore
\def\icrr{1}
\def\ncen{2}
\def\bu{3}
\def\bnl{4}
\def\uci{5}
\def\csu{6}
\def\cnu{7}
\def\duke{8}
\def\gmu{9}
\def\gifu{10}
\def\uh{11}
\def\ui{12}
\def\kek{13}
\def\kobe{14}
\def\kyoto{15}
\def\lanl{16}
\def\lsu{17}
\def\umd{18}
\def\mit{19}
\def\duluth{20}
\def\miyagi{21}
%\def\nagoya{23}
\def\nagoyaste{22}
\def\suny{23}
\def\niigata{24}
\def\okayama{25}
\def\osaka{26}
\def\seoul{27}
%\def\shizuokaseika{28}
\def\shizuoka{28}
\def\shizuokafukushi{29}
\def\skku{30}
\def\tohoku{31}
\def\tokai{32}
\def\tit{33}
\def\tokyo{34}
\def\warsaw{35}
\def\uw{36}
%
\def\corresponding{*}
\def\pennnow{$\dagger$}
\def\kamiokanow{$\ddagger$}
\def\icrrnow{\S}
\def\triumfnow{\P}
\def\stanfordnow{$||$}
\def\columbianow{**}
%\def\corresponding{a}
%\def\pennnow{b}
%\def\kamiokanow{c}
%\def\icrrnow{d}
%\def\triumfnow{e}
%\def\stanfordnow{f}
%\def\columbianow{g}
%
%a hack so things don't take forever to latex
\newcommand{\tempaltaffiltext}[1]{$^{#1}$}
%
\author{
%First author
M.E.C.~Swanson\altaffilmark{\mit,\corresponding},
%Kamioka observatory
K.~Abe\altaffilmark{\icrr}, %not in 3flavor - joined april 2005
J.~Hosaka\altaffilmark{\icrr},
T.~Iida\altaffilmark{\icrr},  %not in 3flavor - joined april 2005
K.~Ishihara\altaffilmark{\icrr},
J.~Kameda\altaffilmark{\icrr},
Y.~Koshio\altaffilmark{\icrr},
A.~Minamino\altaffilmark{\icrr},
C.~Mitsuda\altaffilmark{\icrr},
M.~Miura\altaffilmark{\icrr},
S.~Moriyama\altaffilmark{\icrr},
M.~Nakahata\altaffilmark{\icrr},
%T.~Namba\altaffilmark{\icrr}, %in 3flavor - expired Feb 2006
Y.~Obayashi\altaffilmark{\icrr},
H.~Ogawa\altaffilmark{\icrr},  %not in 3flavor - joined Oct 2004
M.~Shiozawa\altaffilmark{\icrr},
Y.~Suzuki\altaffilmark{\icrr},
A.~Takeda\altaffilmark{\icrr},
Y.~Takeuchi\altaffilmark{\icrr},
K.~Ueshima\altaffilmark{\icrr},  %not in 3flavor- joined april 2005 
%S.~Yamada\altaffilmark{\icrr}, %in 3flavor - expired april 2006
%
%Research center for cosmic neutrinos
I.~Higuchi\altaffilmark{\ncen},
C.~Ishihara\altaffilmark{\ncen}, %not in 3flavor - joined april 2005
M.~Ishitsuka\altaffilmark{\ncen},
T.~Kajita\altaffilmark{\ncen},
K.~Kaneyuki\altaffilmark{\ncen},
G.~Mitsuka\altaffilmark{\ncen},
S.~Nakayama\altaffilmark{\ncen},
H.~Nishino\altaffilmark{\ncen},
A.~Okada\altaffilmark{\ncen}, %in 3flavor - expired april 2006 but contributed to UHE analysis
K.~Okumura\altaffilmark{\ncen},
C.~Saji\altaffilmark{\ncen},
Y.~Takenaga\altaffilmark{\ncen},
%
%Boston U
S.~Clark\altaffilmark{\bu},
S.~Desai\altaffilmark{\bu,\pennnow},
F.~Dufour\altaffilmark{\bu},  %not in 3flavor - joined april 2005
E.~Kearns\altaffilmark{\bu},
S.~Likhoded\altaffilmark{\bu},
M.~Litos\altaffilmark{\bu}, %not in 3flavor - joined april 2005
J.L.~Raaf\altaffilmark{\bu}, %not in 3flavor - joined april 2005
J.L.~Stone\altaffilmark{\bu},
L.R.~Sulak\altaffilmark{\bu},
W.~Wang\altaffilmark{\bu},
%
%BNL
M.~Goldhaber\altaffilmark{\bnl},
%
%Irvine
D.~Casper\altaffilmark{\uci},
J.P.~Cravens\altaffilmark{\uci},
J.~Dunmore\altaffilmark{\uci},  %not in 3flavor - joined june 2004
W.R.~Kropp\altaffilmark{\uci},
D.W.~Liu\altaffilmark{\uci},
S.~Mine\altaffilmark{\uci},
C.~Regis\altaffilmark{\uci},
M.B.~Smy\altaffilmark{\uci},
H.W.~Sobel\altaffilmark{\uci},
%C.W.~Sterner\altaffilmark{\uci}, %in 3flavor - expired 0 2005 ???
M.R.~Vagins\altaffilmark{\uci},
%
%CSU
K.S.~Ganezer\altaffilmark{\csu},
J.E.~Hill\altaffilmark{\csu},
W.E.~Keig\altaffilmark{\csu},
%
%Chonnam National University
J.S.~Jang\altaffilmark{\cnu},
J.Y.~Kim\altaffilmark{\cnu},
I.T.~Lim\altaffilmark{\cnu},
%
%Duke
K.~Scholberg\altaffilmark{\duke,\mit},
N.~Tanimoto\altaffilmark{\duke},  %not in 3flavor - joined april 2005
C.W.~Walter\altaffilmark{\duke},
R.~Wendell\altaffilmark{\duke},  %not in 3flavor - not on ``all'' author list
%
%George Mason U
R.W.~Ellsworth\altaffilmark{\gmu},
%
%Gifu U
S.~Tasaka\altaffilmark{\gifu},
%Hawaii U
G.~Guillian\altaffilmark{\uh},
%A.~Kibayashi\altaffilmark{\uh}, %in 3flavor - expired oct 2005
J.G.~Learned\altaffilmark{\uh},
S.~Matsuno\altaffilmark{\uh},
%
%Indiana University
M.D.~Messier\altaffilmark{\ui},
%KEK
Y.~Hayato\altaffilmark{\kek,\kamiokanow},
A.K.~Ichikawa\altaffilmark{\kek},
T.~Ishida\altaffilmark{\kek},
T.~Ishii\altaffilmark{\kek},
T.~Iwashita\altaffilmark{\kek},
T.~Kobayashi\altaffilmark{\kek},
T.~Nakadaira\altaffilmark{\kek},
K.~Nakamura\altaffilmark{\kek},
K.~Nitta\altaffilmark{\kek},
Y.~Oyama\altaffilmark{\kek},
Y.~Totsuka\altaffilmark{\kek,\icrrnow},
%
%Kobe U
A.T.~Suzuki\altaffilmark{\kobe},
%
%Kyoto
M.~Hasegawa\altaffilmark{\kyoto},
K.~Hiraide\altaffilmark{\kyoto},  %not in 3flavor - joined april 2005
I.~Kato\altaffilmark{\kyoto,\triumfnow},
H.~Maesaka\altaffilmark{\kyoto},
T.~Nakaya\altaffilmark{\kyoto},
K.~Nishikawa\altaffilmark{\kyoto},
T.~Sasaki\altaffilmark{\kyoto},
H.~Sato\altaffilmark{\kyoto},
S.~Yamamoto\altaffilmark{\kyoto},
M.~Yokoyama\altaffilmark{\kyoto},
%
%Los Alamos
T.J.~Haines\altaffilmark{\lanl,\uci},
%
%LSU
S.~Dazeley\altaffilmark{\lsu},
S.~Hatakeyama\altaffilmark{\lsu},
R.~Svoboda\altaffilmark{\lsu},
%
%Maryland U
%E.~Blaufuss\altaffilmark{\umd}, %in 3flavor - expired april 2006
%J.A.~Goodman\altaffilmark{\umd}, %in 3flavor - expired april 2006
G.W.~Sullivan\altaffilmark{\umd},
D.~Turcan\altaffilmark{\umd},
%
% MIT
J.~Cooley\altaffilmark{\mit,\stanfordnow}, %in 3flavor -expired oct 2005 but contributed to UHE analysis
K.B.M.~Mahn\altaffilmark{\mit,\columbianow}, %MIT undergrad who contributed to UHE analysis
%
%University of Minnesota, Duluth
A.~Habig\altaffilmark{\duluth},
%
% Miyagi U. of Education
Y.~Fukuda\altaffilmark{\miyagi}, 
T.~Sato\altaffilmark{\miyagi}, 
%
%Nagoya U.
Y.~Itow\altaffilmark{\nagoyaste},
T.~Koike\altaffilmark{\nagoyaste}, %not in 3flavor - joined april 2005
%
%SUNY
C.K.~Jung\altaffilmark{\suny},
T.~Kato\altaffilmark{\suny},
K.~Kobayashi\altaffilmark{\suny},
M.~Malek\altaffilmark{\suny},
%C.~Mauger\altaffilmark{\suny}, %in 3flavor - expired dec 2005
C.~McGrew\altaffilmark{\suny},
A.~Sarrat\altaffilmark{\suny},
R.~Terri\altaffilmark{\suny}, %not in 3flavor - joined oct 2004
C.~Yanagisawa\altaffilmark{\suny},
%%
%Niigata U
N.~Tamura\altaffilmark{\niigata},
%
%Okayama U.
M.~Sakuda\altaffilmark{\okayama},
M.~Sugihara\altaffilmark{\okayama},%not in 3flavor - joined april 2005
%
%Osaka U.
Y.~Kuno\altaffilmark{\osaka},
M.~Yoshida\altaffilmark{\osaka},
%
%Seoul
S.B.~Kim\altaffilmark{\seoul},
B.S.~Yang\altaffilmark{\seoul},%not in 3flavor - joined march 2005
J.~Yoo\altaffilmark{\seoul},
%
%Shizuoka
T.~Ishizuka\altaffilmark{\shizuoka},
%
%Shizuoka seika
H.~Okazawa\altaffilmark{\shizuokafukushi}, 
%
%Sungkyunkwan University
Y.~Choi\altaffilmark{\skku},
H.K.~Seo\altaffilmark{\skku},
%
%Tohoku U.
Y.~Gando\altaffilmark{\tohoku},
T.~Hasegawa\altaffilmark{\tohoku},
K.~Inoue\altaffilmark{\tohoku},
%J.~Shirai\altaffilmark{\tohoku}, %in 3flavor - expired april 2006
%A.~Suzuki\altaffilmark{\tohoku}, %in 3flavor - expired april 2006
%
%Tokai U
H.~Ishii\altaffilmark{\tokai},%not in 3flavor - joined april 2005
K.~Nishijima\altaffilmark{\tokai},
%
%TIT
H.~Ishino\altaffilmark{\tit},
Y.~Watanabe\altaffilmark{\tit},
%
%Tokyo U
M.~Koshiba\altaffilmark{\tokyo},
%
%Warsaw U
D.~Kielczewska\altaffilmark{\warsaw,\uci},
J.~Zalipska\altaffilmark{\warsaw},
%U Washington
H.G.~Berns\altaffilmark{\uw},
R.~Gran\altaffilmark{\uw,\duluth},
K.K.~Shiraishi\altaffilmark{\uw},
A.~Stachyra\altaffilmark{\uw},%in 3flavor - expired dec 2005 but contributed to UHE analysis
E.~Thrane\altaffilmark{\uw},%not in 3flavor - joined oct 2004
K.~Washburn\altaffilmark{\uw},
and
R.J.~Wilkes\altaffilmark{\uw}\\
(The Super-Kamiokande Collaboration)\\
\footnotesize
\rm
\tempaltaffiltext{\icrr}{Kamioka Observatory, Institute for Cosmic Ray Research, 
University of Tokyo, Kamioka, Gifu, 506-1205, Japan }\\
\tempaltaffiltext{\ncen}{Research Center for Cosmic Neutrinos, Institute for Cosmic 
Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan }\\
\tempaltaffiltext{\bu}{Department of Physics, Boston University, Boston, MA 02215, 
USA }\\
\tempaltaffiltext{\bnl}{Physics Department, Brookhaven National Laboratory, Upton, 
NY 11973, USA }\\
\tempaltaffiltext{\uci}{Department of Physics and Astronomy, University of 
California, Irvine, Irvine, CA 92697-4575, USA }\\
\tempaltaffiltext{\csu}{Department of Physics, California State University, 
Dominguez Hills, Carson, CA 90747, USA }\\
\tempaltaffiltext{\cnu}{Department of Physics, Chonnam National University, Kwangju 
500-757, Korea }\\
\tempaltaffiltext{\duke}{Department of Physics,Duke University, Durham, NC 27708, USA }\\
\tempaltaffiltext{\gmu}{Department of Physics, George Mason University, Fairfax, VA 
22030, USA }\\
\tempaltaffiltext{\gifu}{Department of Physics, Gifu University, Gifu, Gifu 
501-1193, Japan }\\
\tempaltaffiltext{\uh}{Department of Physics and Astronomy, University of Hawaii, 
Honolulu, HI 96822, USA }\\
\tempaltaffiltext{\ui}{Department of Physics, Indiana University, Bloomington,
 IN 47405-7105, USA }\\ 
\tempaltaffiltext{\kek}{High Energy Accelerator Research Organization (KEK), 
Tsukuba, Ibaraki 305-0801, Japan }\\
\tempaltaffiltext{\kobe}{Department of Physics, Kobe University, Kobe, Hyogo 
657-8501, Japan }\\
\tempaltaffiltext{\kyoto}{Department of Physics, Kyoto University, Kyoto 606-8502, 
Japan }\\
\tempaltaffiltext{\lanl}{Physics Division, P-23, Los Alamos National Laboratory, Los 
Alamos, NM 87544, USA }\\
\tempaltaffiltext{\lsu}{Department of Physics and Astronomy, Louisiana State 
University, Baton Rouge, LA 70803, USA }\\
\tempaltaffiltext{\umd}{Department of Physics, University of Maryland, College Park, 
MD 20742, USA }\\
\tempaltaffiltext{\mit}{Department of Physics, Massachusetts Institute of 
Technology, Cambridge, MA 02139, USA }\\
\tempaltaffiltext{\duluth}{Department of Physics, University of Minnesota, 
Duluth, MN 55812-2496, USA }\\
\tempaltaffiltext{\miyagi}{Department of Physics, Miyagi University of Education, Sendai,Miyagi 980-0845, Japan }\\
%\tempaltaffiltext{\nagoya}{Department of Physics, Nagoya University, Nagoya, Aichi 
%464-8602, Japan }\\
\tempaltaffiltext{\nagoyaste}{Solar-Terrestrial Environment Laboratory, Nagoya University, Nagoya, Aichi 464-8601, Japan }\\
\tempaltaffiltext{\suny}{Department of Physics and Astronomy, State University of 
New York, Stony Brook, NY 11794-3800, USA }\\
\tempaltaffiltext{\niigata}{Department of Physics, Niigata University, Niigata, 
Niigata 950-2181, Japan }\\
\tempaltaffiltext{\okayama}{Department of Physics, Okayama University, Okayama, Okayama 700-8530, Japan }\\
\tempaltaffiltext{\osaka}{Department of Physics, Osaka University, Toyonaka, Osaka 
560-0043, Japan }\\
\tempaltaffiltext{\seoul}{Department of Physics, Seoul National University, Seoul 
151-742, Korea }\\
%\tempaltaffiltext{\shizuokaseika}{International and Cultural Studies, Shizuoka Seika College, Yaizu, Shizuoka, 425-8611, Japan }\\
\tempaltaffiltext{\shizuoka}{Department of Systems Engineering, Shizuoka University, 
Hamamatsu, Shizuoka 432-8561, Japan }\\
\tempaltaffiltext{\shizuokafukushi}{Department of Informatics in
Social Welfare, Shizuoka University of Welfare, Yaizu, Shizuoka 425-8611, Japan }\\
\tempaltaffiltext{\skku}{Department of Physics, Sungkyunkwan University, Suwon 
440-746, Korea }\\
\tempaltaffiltext{\tohoku}{Research Center for Neutrino Science, Tohoku University, 
Sendai, Miyagi 980-8578, Japan }\\
\tempaltaffiltext{\tokai}{Department of Physics, Tokai University, Hiratsuka, 
Kanagawa 259-1292, Japan }\\
\tempaltaffiltext{\tit}{Department of Physics, Tokyo Institute for Technology, 
Meguro, Tokyo 152-8551, Japan }\\
\tempaltaffiltext{\tokyo}{The University of Tokyo, Tokyo 113-0033, Japan }\\
\tempaltaffiltext{\warsaw}{Institute of Experimental Physics, Warsaw University, 
00-681 Warsaw, Poland }\\
\tempaltaffiltext{\uw}{Department of Physics, University of Washington, Seattle, WA 
98195-1560, USA }
%end authors
}
\altaffiltext{\corresponding}{Electronic address: molly@space.mit.edu}
\altaffiltext{\pennnow}{Present address: Center for Gravitational Wave Physics, Pennsylvania State University, University Park, PA 16802, USA}
\altaffiltext{\kamiokanow}{Present address: Kamioka Observatory, Institute for Cosmic Ray Research, University of Tokyo, Kamioka, Gifu, 506-1205, Japan}
\altaffiltext{\icrrnow}{Present address: Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Chiba 277-8582, Japan}
\altaffiltext{\triumfnow}{Present address: TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\altaffiltext{\stanfordnow}{Present address: Department of Physics, Stanford University, Stanford, CA 94305, USA}
\altaffiltext{\columbianow}{Present address: Department of Physics, Columbia University, New York, NY 10027, USA}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

